A new solution to the curved Ewald sphere problem for 3D image reconstruction in electron microscopy

We develop an algorithm capable of imaging a three-dimensional object given a collection of two-dimensional images of that object that are significantly influenced by the curvature of the Ewald sphere. These two-dimensional images cannot be approximated as projections of the object. Such an algorithm is useful in cryo-electron microscopy where larger samples, higher resolution, or lower energy electron beams are desired, all of which contribute to the significance of Ewald curvature.

==> Makefile <==
FILE=paper1

SRC=\
   $(FILE).tex

$(FILE).pdf: $(SRC)
	pdflatex $(FILE)
	bibtex $(FILE)
	pdflatex $(FILE)
	pdflatex $(FILE)

clean:
	rm -f *.nav *.toc *.out *.snm *.aux *.log
	rm -f *.bbl *.blg *.spl

distclean:
	rm -f *.nav *.toc *.out *.snm *.aux *.log $(FILE).pdf
	rm -f *.bbl *.blg *.spl

tar:
	tar -czf $(FILE).tgz $(FILE).tex $(FILE).bib $(FILE).bbl *.png algo.pdf model5-names.bst Makefile


